Benchmarks for Pir\'a 2.0, a Reading Comprehension Dataset about the Ocean, the Brazilian Coast, and Climate Change

Pir\'a is a reading comprehension dataset focused on the ocean, the Brazilian coast, and climate change, built from a collection of scientific abstracts and reports on these topics. This dataset represents a versatile language resource, particularly useful for testing the ability of current machine learning models to acquire expert scientific knowledge. Despite its potential, a detailed set of baselines has not yet been developed for Pir\'a. By creating these baselines, researchers can more easily utilize Pir\'a as a resource for testing machine learning models across a wide range of question answering tasks. In this paper, we define six benchmarks over the Pir\'a dataset, covering closed generative question answering, machine reading comprehension, information retrieval, open question answering, answer triggering, and multiple choice question answering. As part of this effort, we have also produced a curated version of the original dataset, where we fixed a number of grammar issues, repetitions, and other shortcomings. Furthermore, the dataset has been extended in several new directions, so as to face the aforementioned benchmarks: translation of supporting texts from English into Portuguese, classification labels for answerability, automatic paraphrases of questions and answers, and multiple choice candidates. The results described in this paper provide several points of reference for researchers interested in exploring the challenges provided by the Pir\'a dataset.

==> at.tex <==
\section{Answer Triggering}

%%%%%%%%%%%%%%
% Talvez abordar como um problema de answer triggering não seja o melhor. Outra possibilidade é abordar como uma tarefa de distinguir entre questões bem-feitas e mal-feitas, entre questões válidas e inválidas.
%%%%%%%%%%%%%%

Generally, a QA system is thought as a conditional generator which predicts an answer given a question. The main goal of QA systems is to answer questions given by users, usually over some limited subject. A QA system can be considered better, therefore, when the answers it generates are more adequate according to some measure (e.g., ground truth answers, internal consistency, etc.).

In practice, however, it is unlikely that a particular QA system is able to answer any possible question; or, even, any question put by its users in practice (unless questions take a very strict closed format). The reasons for that go from the lack of necessary information, to malformed questions, ambiguity, non-shared assumptions, among others. 

In some cases, giving an answer may be better than no answer at all; or at least, better in general (assuming a high accuracy rate for the model). In other cases, however, providing a wrong answer may have dangerous consequences. Suppose a QA system that conducts a preliminary medical sorting; given the symptoms of the patient, the system tells what problems they could have, if any, and what kind of doctor they should look for. Informing a person that they have a disease when they do not, or diagnosing them with a wrong disease, may provoke serious damages. Individuals could initiate self-medication medication, delay appropriate treatment, not counting the psychological damages depending on the diagnosis. Instead of wrongly answering such question, it would be better that the QA system avoided answering at that question at all, unless it was strongly certain of it.\footnote{There is also a large literature on the harmful impacts language models can have on bias amplification and toxicity \cite{weidinger2021ethical}. In this paper, we consider the more limited problem of low quality answers as regards to meaningfulness.}

In sum, it is important that a system knows \textit{when} it should answer a question. This is important to guarantee safety (i.e., consistency with human values) and factual grounding \cite{thoppilan2022lamda}.
% In other words, a QA system should understand when it should be triggered or not. 
Answer triggering is precisely the task of deciding when a question should be answered or not. By allowing some questions not to have an answer, models are required to learn when they are able to answer a given question, a task known as “answer triggering”. The task become popular with SQuAD 2.0 \cite{rajpurkar2018know}). 
% 3-point uncertainty scale

It is possible to distinguish two kinds of questions that do not have answer: unanswerable and invalid questions \cite{rogers2021qa}. The former are questions that cannot be answered given all the information the reader have access to, and the latter are questions that a speaker would reject to answer. Similarly, we could think of unanswerable questions are those that cannot be answered by the available evidence (context, common sense, preceding information, etc.), whereas invalid questions cannot be answered with any amount of evidence, because they are grounded on invalid premises, are grammatically ill-formed, among other possible causes. For our task, we ignore this distinction, since we want to test the ability to recognize questions that should not be answered for whatever reason. In other words, what call ``unanswerable'' questions encompass both properly unanswerable question as well as wrongly put questions. One reason to ignore this is that, although it makes sense analytically, the distinction is rather vague in practice. Also, Pirá does not permit to distinguish question in this way. Finally, in both cases, the goal is the same: prevent the system of answering some questions.

%%%%%%%%%
% Hipótese para testar se as perguntas são inválidas ou sem resposta, on sentido tradicional. Se as perguntas forem inválidas, talvez o input com apenas a questão produza resultados melhores. Isso porque o problema estaria na maneira como a pergunta é feita (essa é uma das possibilidades, de perguntas mal-feita, mas outras formas de invalidez são possíveis). Nesse caso, a adição do abstract só traria ruídos. 
%%%%%%%%

\subsection{Classification}
In SQuAD 2.0, unanswerable questions were constructed by crowdworkers with that purpose in sight. Annotators were asked to create questions over paragraphs that could not be correctly answered with from that piece of text only. To avoid that questions unrelated to the context were created, the authors instructed the annotators to produce questions that were relevant to the context and which contained plausible answers in the paragraph (such as the name of a person for a Who-type question).

\textit{Pirá} does not contain intentionally produced unanswarable questions. All questions in the dataset are paired with their respective answers. Instead, we use information provided in the assessment phase to select unanswerable questions. When evaluating the QA sets created in the first phase, volunteers had to evalute if QA sets were meaningful, according to a Likert scale (1 - Strongly disagree, 2 - Disagree, 3 - Neither agree nor disagree, 4 - Agree, 5 - Strongly agree). We thus take question meaninglessness as a proxy for unanswerability. We consider that questions that are not meaningful cannot be answered.

% The converse, however, is not necessarily true: a question may be meaningful an yet unanswerable. Hence, we use another assessment that was produced by volunteers to filter answerable questions among the meaningful ones: we only take those that received a ``Yes'' for the question ``Can you answer the question only with the information provided by the text?''.

The aim of answer triggering is to predict whether a question has an answer or not. As for the classification label, we considered the evaluation of question meaningfulness. Therefore, this is therefore a binary classification task where 1 means that a question has an answer and 0 that it has not.

We consider here three baselines. The first was a Yes-to-all model. For all questions, the model attributed 1. We believe this offers a strong baseline, considering that human evaluations strongly leaned to meaningfulness. To perform better than that, a model needs to realize subtle elements that indicate unanswerability. 

Following \cite{jose2022}, we consider then approaches that represent successive degrees of complexity. The second baseline in our list was a Naive Bayes approach. Naive Bayes is a classifier that assumes independence between words. This method is useful in discriminating topics and sentiment analysis, since classes in those tasks can be often determined by word frequency. We use Naive Bayes as a baseline for measuring how much answer triggering is dependent on co-occurrence of words. If this algorithm performs well, there is evidence that unanswerability can be detected by the presence of specific words.

Finally, we considered also a transformer-based approach. This offers a much more sophisticated strategy, where word order is taken into account and where tokens have dense representations. We run the model for 8 epochs and chose the model that achieved the lowest loss in the validation set, and used that model in the test set. For English, we used RoBERTA \cite{liu2019roberta}, which is a BERT architecture \cite{devlin2018bert} trained on additional data and optimized as regards its hyperparameters. For Portuguese, we used BERTimbau \cite{souza2020bertimbau}, a pretrained BERT model for Brazilian Portuguese.

In addition, we wanted to analyze if the results were homogeneous, or differed depending on the language, corpora, context, or any other variable. For that reason, we run tests for a number of combinations, totaling 216 scenarios. Six parameters were assessed:

\begin{enumerate}
    \item \textbf{Language:} English, Portuguese.
    \item \textbf{Corpus:} Full, UN reports, articles.
    \item \textbf{Context:} Question+abstract, question, abstract.
    \item \textbf{Data:} Standard, human paraphrases, automatic paraphrases.
    \item \textbf{Balancing:} Balanced, unbalanced.
    \item \textbf{Label classification:} Strong, weak.
\end{enumerate}

\textbf{Language:} Pirá is a bilingual dataset. We separately tested the classification models on Portuguese and English.

\textbf{Corpus:} Two corpora were employed as a source of context for the creation of questions: scientific abstracts on the Brazilian Coast and two reports on the ocean conducted by the United Nations. We run the tests for each of the corpora separated, as well as for the full corpus.

\textbf{Context:} Ideally, the questions in Pirá should demand that someone consulted both the question and the abstract to be answered, since it was planned as a reading comprehension dataset. It is known, however, that artifact annotations can sometimes provide clues, imperceptible to human beings but detectable by neural models, on how to solve a certain task \cite{gururangan2018annotation}. Analogously, we wanted to test if our answering triggering task could be solved by only having the question or the abstract as input, or if both were necessary to determine answerability.

\textbf{Data:} The standard version of Pirá 2.0 contains 2248 QA sets. In addition to that, we produced two extended version of the dataset, given that only a few QA sets had a low evaluation. First, we considered the validation answers and paraphrased questions produced in the assessment phrase. We combined them with the original questions and answers, and formed an extended version of the dataset based on the human paraphrases. Hence, a single question-answer pair was replaced for up to four pairs: original question - original answer; original question - validation answer; paraphrased question - original answer; paraphrased question - paraphrased answer.\footnote{Not all questions have paraphrases, since this was an optional step. In total, 1965 (86.0\%) of the questions were paraphrased. All QA sets that passed for the assessment phase (2187 or 96.8\%) have a validation answer.} Second, we also created an expanded version of Pirá based on automatic paraphrasers. For every original question, we generated up to 5 paraphrased questions, and did the same for the original answers. See Table \ref{tab:QAexample} for some examples of automatic paraphrases. After doing that, we combined the various the various questions and answers in pairs, as we did for the human paraphrases. For English, we used PEGASUS \cite{zhang2020pegasus}, a state-of-the-art self-supervised transformer model designed for abstractive summarization, fine-tuned for paraphrasing.\footnote{https://huggingface.co/tuner007/pegasus\_paraphrase.} We also experimented a T5 model fine-tuned on Tapaco, a dataset for paraphrase generation \cite{raffel2019exploring}, but the results were not so satisfactory.\footnote{https://huggingface.co/hetpandya/t5-small-tapaco} For Portuguese, we employed the Portuguese version of the original T5 architecture, PTT5 \cite{carmo2020ptt5}, fine-tuned on the Portuguese part of the Tapaco \cite{pellicer2022}.

\begin{table*} [tp]
  \caption{Example of automatic paraphrases}
  \label{tab:QAexample}
  \begin{tabular}{p{1.5cm}p{5cm}p{5cm}}
    \toprule
    Language & Original question & Automatic Paraphrase\\
    \midrule
    \\ 
    English & \small{\textbf{Question:} When did the first phase of the development plan conceived for Albacora field start? [ID A775]} \newline \newline \newline \newline \newline \newline \newline  \textbf{Answer:} Mature regions, such as the North Sea and the Gulf of Mexico. [ID B2062] & \footnotesize{When did the first phase of the program, which was intended for Albacora field, begin?} \newline When did the start of the first phase of the study of Albacora field's field plan? \newline When did the first phase of the development plan for the field for Albaniacora? \newline When did the first phase of the development plan, designed for Albacora field, start? \newline When did the first phase of the project conceived for the Albacora field field start? \newline \newline Mature areas such as the North Sea or the Gulf of Mexico are all covered. \newline Some regions are called the North Sea and the Gulf of Mexico. \newline Motherlands like the North Sea and the Gulf of Mexico are thriving. \newline Mature regions include the North Sea and the Gulf of Mexico. \newline Mature regions such as North Sea and Gulf of Mexico. \newline\\ Portuguese & \small{\textbf{Question:} Onde podemos achar locais de nascimento de C. limbatus? [ID A1217]} \newline \newline \newline \newline \newline \newline \textbf{Answer:} Devido à magnitude da propagação vertical de energia e duração dos eventos. [ID A1942] & \footnotesize{Onde se pode encontrar a localização da família de C. limbatus? \newline Onde podemos achar locais de nascimento de C. limbatus? \newline Onde podemos encontrar a localização do berço do mosquito do nome? \newline Onde podemos encontrar o local de nascimento de C. limbatus? \newline Onde poderíamos encontrar locais de nascimento do C. limbatus? \newline \newline Isso é devido à intensidade da transmissão vertical de energia e à duração dos eventos. \newline Devido à intensidade de propagação vertical de energia e a duração de eventos. \newline Por causa da grande quantidade de energia transmitida verticalmente e da duração dos eventos. \newline A intensidade de onda vertical é determinada pela intensidade da onda vertical e pela duração das ondas. \newline Isto é devido à intensidade de propagação vertical de energia e à duração dos eventos.}\\
    \bottomrule
  \end{tabular}
\end{table*}

\textbf{Balancing:} Pirá is heavily unbalanced as regards to question meaningfulness, with a much larger number of questions in the meaningful side. (Figure~\ref{fig:merged_QA_meaning}) shows similar distribution as regards question meaningfulness in the training, validation, and test set, for a standard combination of parameters.\footnote{Test number 1: [language = `English'; corpus = `full'; context = `question+abstract', data = `standard', balancing = `balanced', label classification = `soft'].} For this reason, we also considered balanced version of the dataset, in which we undersampled the larger classes, using a number of observations for each group (1-5) in the training equal to that of the smallest group. Validation and test sets were not balanced. Both balanced and unbalanced versions of the dataset were tested.

\textbf{Label Classification:} As said, unanswarable questions were not intentionally created in Pirá, but assumed based on the assessments produced in phase two of the dataset generation process. For that, we considered the evaluations of meaningfulness. In the weak version, all questions that received 3-5 were labeled answerable and those receiving 1-2 as unanswerable. In the strong version, only questions that obtained 1 or 5 were used, disregarding intermediate scores. That was the only parameter which had impĺications to the test set, since question meaningfulness (as a binary outcome) was not an original property of the dataset; in the case of strong versions of the dataset, we limited our test set to scores 1 and 5. We applied the same policy to the validation set.

\subsubsection{Results}
Each combination of parameters formed a specific test, which led to different results. For instance, in test 1 [language = `English'; corpus = `full'; context = `question+abstract', data = `standard', balancing = `balanced', label classification = `weak'], the number of QA sets (after excluding those without assessment) was 1755 for training, 215 for validation, and 216 for test. After balancing, all groups were cut at the size of the smallest group; in this case, 49. The majority of questions in each question were answerable. Table \ref{tab:test_1} brings a summary of the training data of this test.

As emphasized, results differed depending on the particular values taken by the hyperparameters. Nonetheless, some general. Tables ~\ref{tab:results_classifiers_en} and ~\ref{tab:results_classifiers_pt} summarize the results for the tests in the English and Portuguese, respectively. Maximum, minimum and average values are provided for accuracy and f1-score. \textbf{Appendix A} brings the detailed results for all the tests.

\begin{table}[h]
\caption{Results of classifiers in English. Every cell presents mean, min, and max values for accuracy and F1-score. Mean value is in bold.}
\label{tab:results_classifiers_en}
\centering
\begin{tabular}{|l|c|c|}
\hline
{\bf Classifier} & \textbf{Accuracy} & \textbf{F1-score} \\ \hline
Simple assignment & \textbf{0.9225} (0.9120 - 0.9379) & \textbf{0.9596} (0.9539 - 0.9679) \\ \hline
Naive Bayes & \textbf{0.8224} (0.2551 - 0.9379) & \textbf{0.8236} (0.3420 - 0.9078) \\ \hline
Transformer (RoBERTA) & \textbf{0.8730} (0.0620 - 0.9379) & \textbf{0.9388} (0.6372 - 0.9679)\\ \hline
\end{tabular}
\end{table}

\begin{table}[h]
\caption{Results of classifiers in Portuguese. Every cell presents mean, min, and max values for accuracy and F1-score. Mean value is in bold.}
\label{tab:results_classifiers_pt}
\centering
\begin{tabular}{|l|c|c|}
\hline
{\bf Classifier} & \textbf{Accuracy} & \textbf{F1-score} \\ \hline
Simple assignment & \textbf{0.9120} (0.9120 - 0.9120) & \textbf{0.9539} (0.9539 - 0.9539) \\ \hline
Naive Bayes & \textbf{0.8175} (0.2037 - 0.9120) & \textbf{0.8115} (0.2324 - 0.8762) \\ \hline
Transformer (BERTimbau) & \textbf{0.8649} (0.3703 - 0.9120) & \textbf{0.9239} (0.5072 - 0.9539)\\ \hline
\end{tabular}
\end{table}

% Teve só alguns casos em que o naive bayes foi melhor que o simple assingment; mas esses foram por uma margem pequena e somente quando o simple assingment não teve valores tão bons.

The accuracy of the simple assignments (saying all questions have answer) ranged from 0.9090 to 0.9127. To beat that, classifiers would have to guess some of the true negatives.

Naive Bayes classifiers were generally not able to overcome this simple assignment. In the best cases (almost a fourth of the tests), Naive Bayes followed the same strategy as simple assignment: it attributed all questions to the answerable class. It did not perform better than simple assingment in any case, for both accuracy and f1-score. When anything other than simple assignment was done, Naive Bayes achieved a performance worse than the first baseline. In addition, it showed much more variability.

Compared to Naive Bayes, the transformer classifier was more consistent. Nonetheless, the higher performance in general was again due to the use of the simple assignment strategy. These models classified all question as answerable in 50.92\% of the cases (110 out of 216), and for this reason achieved a high accuracy and F1-score. Differences were mostly due to the ``balancing'' parameter: 87.96 (95 out of 108) of the balanced tests opted exclusively for the largest class in the classification; whereas only 13.88 of the unbalanced tests (15 out of 108) did the same. In any case, the transformed approach did not beat the simple assignment baseline, be it for accuracy or f1-score, in any test.

\begin{figure*}[tp]
  \centering
  \includegraphics[width=1\textwidth]{images/QA_sets.png}
  \caption{Distribution of evaluations of question meaningfulness in training, validation and test set for Test 1.}
  \label{fig:merged_QA_meaning}
\end{figure*}

\begin{table}[h]
\caption{Test number 1}
\label{tab:test_1}
\centering
\begin{tabular}{|l|c|c|c|}
\hline
{\bf Set} & \textbf{Original \#QAs} & \textbf{\#QAs w/ evaluation} & \textbf{Questions w/o answer} \\ \hline
Training   & 1806  & 1755 & 137/98\footnote{We filtered QAs that were considered meaningful but could not be answered by the text only. That is why the numbers in this column to not to the values in the column in the left.} \\ \hline
Validation    & 225  & 215 & 195/19 \\ \hline
Test   & 227 & 216 & 191/19 \\ \hline
\end{tabular}
\end{table}


\subsection{Regression task}
Overall, our classifiers have failed in the answer triggering task --- they were not able to discriminate between answerable and unasnwerable questions better than a a guess based on class frequency. This may be seen as an evidence that ``answerable question" is not a real phenomenon or that Pirá is poorly marked. In this section, we decided to perform a related task, that we called \textit{continuous answer triggering} (CAT). CAT is a regression task, in which we aim to predict the degree of question meaningfulness in a scale; something which, if successful, may indicate that the task of identifying answerability, although subtle, is possible at some level.

Part of the problem of the classification task, we believe, derives from the fact that answerability is not a binary variable. Although a many questions can be undoubtedly categorized as meaningful or meaningless, other questions may lay in the middle part of the meaningfulness spectrum. Some reading comprehension datasets try to overcome this difficulty by including a third outcome signaling uncertainty as another possible outcome. ReCO \cite{wang2020reco}, a dataset of opinion based queries in Chinese, uses three candidate answers for annotation: a positive one like Yes, a negative one like No, and an undefined one if the question could not be answered with the given documents. QuAIL \cite{rogers2020getting}, a multi-choice dataset, is developed to include three degrees of certainty: answerable questions (given a context), unanswerable questions (even with context and world knowledge), and partially certain questions (when a good guess can be made).

Contrary to this datasets, Pirá does not posses an explicitly features indicating unswerability or certainty degree. The human evaluations conducted in the assessment, nonetheless, allow us to infer this type of information present in the questions. The Likert scale (1-5) used in the evaluations provides a fine-grained analysis of the answerability of questions, more so than a binary or three-point alternative; even better, it permits us to treat question meaningfulness as a ordinal variable. 

Based on that, we reframed our answer triggering problem as a regression task. The problem now is that of estimating the meaningfulness of a question, so as to inform a decision on answerability. As in the classification task, we used the transformer based approach RoBERTA for English and BERTimbau for Portuguese. We experimented with the same grid of hyperparameters, leading to 54 different tests (half in English, half in Portuguese).\footnote{Because there is no ``label classification'' in this task, the number of combinations is half of the classification task.} In each case we run the regression model for 8 epochs, saving the best model according to validation set's loss. We then chose the combination of hyperparameters that achieved the best according to this metric.

\subsubsection{Regression filtering in English}
Although, our regressor was not always successful in predicting meaningfulness, we wanted to test if, in the best case, the regressor could help to filter out unanswerable questions. If true, then a QA system that predicted the meaningfulness of questions and chose to answer only the better ones could give superior answers overall. 

In order to test that, we used the combination of hyperparameters that engendered the smallest loss in the validation test: (language = `english'; corpus = `articles'; context = `abstract', data = `standard', balancing = `unbalanced')[test 171]. In our experiments, validation loss ranged from a minimum of 0.0705 to a maximum of 0.1664, with an average value of 0.0948.

In another way to measure the quality of the regressions, we used the R-squared metrics. While multiclass transformer regressor employs cross entropy loss, R-squared is based on the mean squared error. In our case, the mean value used for computation was obtained from the validation set, in order to assess the improvements in error reduction provided by the prediction as compared to a simple estimate of the mean value of the validation set. More formally, where $\bar{y}$ is the average evaluation of meaningfulness in the validation set, R-square was defined as:

\begin{equation}
R^2 = 1 - \frac{\sum_{1}^{n}(y_i - \widehat{y_i})^2}{\sum_{1}^{n}(y_i - \bar{y}_{validation})^2}
\end{equation}

Contrary to evaluation loss, we want to maximize the value of R-squared. In our experiments, R-squared highly coincided in the ranking with the evaluation loss metric, including for the first 20 results. R-squared ranged from -1.3394 to 0.0043, with a mean value of -0.3365. Again, test 171 occupied the first position (Table \ref{tab:correlation_en}). For this reason, we decided to use this combination of hyperparameters as input to the QA system.

\begin{table}[h]
\caption{Top results of the regression tests in English}
\label{tab:correlation_en}
\centering
\begin{tabular}{|l|c|c|c|}
\hline
\textbf{Ranking} & \textbf{Test number} & {\bf Validation loss}   & \textbf{R-squared} \\ \hline
1 & 171 & 0.0705 & 4.3752e-03 \\ \hline
2 & 151 & 0.0707 & 2.1338e-03 \\ \hline
3 & 139 & 0.0708 & 2.2967e-05 \\ \hline
4 & 163 & 0.0708 & -4.7841e-05 \\ \hline
5 & 159 & 0.0709 & -1.3767e-03 \\ \hline
\end{tabular}
\end{table}

For computational limitations, we were not able to save all models; therefore, we had to rerun the regression again on this particular training set (i.e., test 201) as regards meaningfulness evaluation, using the validation loss to select the best epoch. That model was then used to predict the meaningfulness of questions in the test set. 10 partitions of the dataset based on the quality of the questions according to the regressor were created.

As for the QA system, we used a distilbert model \cite{sanh2019distilbert} (a lighter version of the BERT architecture) fine-tuned for question answering on two reading comprehension datasets: SQuAD 1.1 \cite{rajpurkar2016squad} and SQuAD 2.0 \cite{rajpurkar2018know}. SQuAD 1.1 is a reading comprehension dataset with 100K+ questions with extractive answers. For SQuAD 2.0, 53K questions unanswerable questions were added to the original dataset.

Our first test measured the quality of answers for each partition of the test set. As smaller partitions select questions evaluated better according to our regressor, we would expect that answers generated to them would be better. To measure the quality of answers, we used f1-score. Table \ref{tab:prediction} and Figure \ref{fig:prediction} show the results for both QA models.

\begin{figure*}[tp]
  \centering
  \includegraphics[width=0.9\textwidth]{images/prediction.png}
  \caption{F1-score for different partitions of test set for answers generated with SQuAD 1.1 and SQuAD 2.0, based on predicted values.}
  \label{fig:prediction}
\end{figure*}

\begin{table}[h]
\caption{F1-score for different partitions of test set for answers generated with SQuAD 1.1 and SQuAD 2.0, based on predicted values}
\label{tab:prediction}
\centering
\begin{tabular}{|l|c|c|}
\hline
{\bf Partition}   & \textbf{SQuAD 1.1} & \textbf{SQuAD 2.0}\\ \hline
100	&41.80	&38.87\\ \hline
90	&42.25	&39.83\\ \hline
80	&42.90	&40.87\\ \hline
70	&42.18	&40.73\\ \hline
60	&42.72	&40.17\\ \hline
50	&42.96	&40.14\\ \hline
40	&45.69	&41.43\\ \hline
30	&46.65	&45.24\\ \hline
20	&48.48	&47.17\\ \hline
10	&51.50	&48.12\\ \hline
\end{tabular}
\end{table}

Answers generated with both QA models show a similar trend for SQuAD 1.1 and SQuAD 2.0. In both cases, there is an increase in F1-score when smaller partitions of the original test set feed the QA system. As we will argue later, though, we should be careful when analysing the results for small partitions. In this as in other tests, results for both QA models are similar. This is expected, given the F1-score between the answers generated with these two models of 70.03. In general, though, the F1-score for SQuAD 1.1 is higher than for SQuAD 2.0. 

F1-score is a metric based on the presence of the same tokens in the ground and predicted answers. It is known that automatic metrics may not correlate well with human evaluations \cite{liu2016not}. There is also a more straightforward shortcoming of F1-score: this metric is not able to identify subtler similarity phenomena between answers, involving paraphrasing. For this reason, we wanted to check if this metric was able to capture relative trends in similarity, even if is short of measuring similarity in general. In order to assess that, we used a second metric to check the ability of F1-score to measure similarity, based on vector representations of the answers. Those embeddings were produced with Sentence-BERT \cite{reimers2019sentence}. Cosine dissimilarity (1 - cosine distance) served as a measure of content similarity (rather than word similarity, as in the case of F1-score). Table \ref{tab:distance} and Figure \ref{fig:distance} show the results for both QA models.

\begin{figure*}[tp]
  \centering
  \includegraphics[width=0.9\textwidth]{images/distance.png}
  \caption{Cosine dissimilarity for different partitions of test set for answers generated with SQuAD 1.1 and SQuAD 2.0, based on predicted values.}
  \label{fig:distance}
\end{figure*}

\begin{table}[h]
\caption{Cosine dissimilarity for different partitions of test set for answers generated with SQuAD 1.1 and SQuAD 2.0, based on predicted values}
\label{tab:distance}
\centering
\begin{tabular}{|l|c|c|}
\hline
{\bf Partition}   & \textbf{SQuAD 1.1} & \textbf{SQuAD 2.0}\\ \hline
100	&41.80	&38.87\\ \hline
90	&42.25	&39.83\\ \hline
80	&42.90	&40.87\\ \hline
70	&42.18	&40.73\\ \hline
60	&42.72	&40.17\\ \hline
50	&42.96	&40.14\\ \hline
40	&45.69	&41.43\\ \hline
30	&46.65	&45.24\\ \hline
20	&48.48	&47.17\\ \hline
10	&51.50	&48.12\\ \hline
\end{tabular}
\end{table}

Answer similarity, as measured by the cosine distance of sentence embeddings, tends to fall for smaller partitions, particularly when less than half of the dataset is selected. Before that, results are static for SQuAD 1.1, while SQuAD 2.0 shows a momentary decrease aroung 7080\% of the dataset. An for F1-score, SQuAD 1.1 performs better than SQuAD 2.0 concerning cosine dissimilarity.

Our results for F1-score are considerably worse than the reported in the original papers. According to the authors, a F1-score of 51\% can achieved with a strong logistic regression model for SQuAD 1.1 \cite{rajpurkar2016squad}, and neural models can raise this to 86\% on SQuAD 1.1 and 66\% for SQuAD 2.0, respectively \cite{rajpurkar2018know}. 

Part of problem may be explained by the non-extractive nature of Pirá and the higher difficulty of the supporting texts. Another aspect comes from random elements of the regressor, which despite our use of controlled seeds whenever possible, produces random variations in results.

In addition to these elements, we wanted to explored other possible sources that accounted for the results. A first difficulty could be due to the inaccuracy of our regressor. Therefore, we took the evaluations of question meaningfulness instead of the predictions based on the regressor. Although this information is never present in real applications, this analysis may point to the shortcomings derived from our partitioning process. Table \ref{tab:distance} and Figure \ref{fig:real_value} shows the results for both QA models.

%For SQuAD 1.1 and SQuAD 2.0 there is an increase in the F1-score of smaller and better partitions of the dataset.\footnote{We believe part of the irregular behavior may be due to the ties in the ranking table, which lead to partitions that are not so homogenous.}

\begin{figure*}[tp]
  \centering
  \includegraphics[width=0.9\textwidth]{images/real_value.png}
  \caption{F1-score for different partitions of test set for answers generated with SQuAD 1.1 and SQuAD 2.0, based on true evaluations.}
  \label{fig:real_value}
\end{figure*}

\begin{table}[h]
\caption{F1-score for different partitions of test set for answers generated with SQuAD 1.1 and SQuAD 2.0, based on true evaluations.}
\label{tab:real_value}
\centering
\begin{tabular}{|l|c|c|}
\hline
{\bf Partition}   & \textbf{SQuAD 1.1} & \textbf{SQuAD 2.0}\\ \hline
100	&41.81	&38.87\\ \hline
90	&42.12	&38.35\\ \hline
80	&43.10	&39.54\\ \hline
70	&42.55	&39.75\\ \hline
60	&42.95	&40.40\\ \hline
50	&44.49	&40.12\\ \hline
40	&45.13	&41.55\\ \hline
30	&46.35	&41.58\\ \hline
20	&48.83	&44.92\\ \hline
10	&43.51	&40.62\\ \hline
\end{tabular}
\end{table} 

Two things can be seen from these figures. First, the use of true labels entail a smoother trend, with the F1-score improving for smaller partitions (with the exception of the 10\% partition, but which due to its small size, is not totally representative). Second, in both cases, the F1-score is higher when human evaluations are considered, instead of predicted ones. 

When the F1-score is considered for each true evaluation level, the relation is less clear. This is shown in Figure \ref{fig:real_labels_bar}. It seems counter-intuitive that lower quality questions (according to the annotators' evaluations) achieve higher F1-scores. One reason for that may be a problem with human evaluations, perhaps due to the a fail in with the instructions. However, we must also consider that the small number of examples of low meaning questions, so it is expected that predictions do not be as good for them as for higher values. Arguably, one of the reasons our regressor perform badly is the small number of low meaningfulness questions. Table \ref{tab:labels_size} and Figure \ref{fig:labels_size} show the number of QA sets for each level of evaluation. For the larger group of questions evaluated from 3 to 5, F1-score seems to work as expected.

\begin{table}[h]
\caption{Number of QA sets for evaluation level}
\label{tab:labels_size}
\centering
\begin{tabular}{|l|c|}
\hline
{\bf Label}   & \textbf{Size}\\ \hline
1&	9 (4.1\%)\\ \hline
2&	10 (4.6\%)\\ \hline
3&	18 (8.3\%)\\ \hline
4&	43 (19.9\%)\\ \hline
5&	136 (62.9\%)\\ \hline
\end{tabular}
\end{table}

\begin{figure*}[tp]
  \centering
  \includegraphics[width=0.65\textwidth]{images/labels_size.png}
  \caption{Number of QA sets for different levels of question meaningfulness.}
  \label{fig:labels_size}
\end{figure*}

\begin{figure*}[tp]
  \centering
  \includegraphics[width=0.9\textwidth]{images/real_labels_bar.png}
  \caption{F1-score for different score values, using SQuAD 1.1 and SQuAD 2.0.}
  \label{fig:real_labels_bar}
\end{figure*}


This result is actually expected, when we consider the correlation between predicted and true evaluations of meaningfulness. Table \ref{tab:correlation} and Figure \ref{fig:correlation}(a) present the mean value of the question evaluation for each value of the true label (normalized for the range 0-1). The Pearson correlation for this pair of variables gives a value of 0.0336, with a two-sided p-value of 0.6228. In other words, our regressor only slightly predicts the true meaningfulness of questions and even this without statistical significance. This weak correlation can be also seen in Figure \ref{fig:correlation}(b).



\begin{figure*}[tp]
  \centering
  \includegraphics[width=0.9\textwidth]{images/correlation.png}
  \caption{(a) Correlation between real labels and predictions (line plot); (b) Correlation between real labels and predictions (scatter plot)}
  \label{fig:correlation}
\end{figure*}

\begin{table}[h]
\caption{Mean prediction for true question meaningfulness}
\label{tab:correlation}
\centering
\begin{tabular}{|l|c|}
\hline
{\bf True label}   & \textbf{Mean prediction}\\ \hline
0 &	84.36\\ \hline
0.25 & 84.16\\ \hline
0.5 & 84.19\\ \hline
0.75 & 84.35\\ \hline
1 & 84.31\\ \hline
\end{tabular}
\end{table}


As a final test, we evaluated if part of the explanation for the low F1-score was not also due to the question answering models. Low F1-scores could be due in part to shortcomings of these QA models. In order to assess that, we tested the agreement, measured by F1-score, between answers given in the QA creation phase and those given in the evaluation phrase. Again, we used real assessments of question meaningfulness as the criterion for partitioning the test set. Table \ref{tab:validation} and Figure \ref{fig:validation_answers} present the results for this test.

\begin{figure*}[tp]
  \centering
  \includegraphics[width=0.65\textwidth]{images/validation_answers.png}
  \caption{F1-score for different partitions of test set for validation answers, based on true evaluations.}
  \label{fig:validation_answers}
\end{figure*}

\begin{table}[h]
\caption{F1-score for different partitions of test set for validation answers, based on true evaluations}
\label{tab:validation}
\centering
\begin{tabular}{|l|c|}
\hline
{\bf Partition}   & \textbf{F1-score}\\ \hline
100	&54.85\\ \hline
90	&56.69\\ \hline
80	&58.86\\ \hline
70	&58.83\\ \hline
60	&59.19\\ \hline
50	&60.75\\ \hline
40	&62.31\\ \hline
30	&61.77\\ \hline
20	&61.08\\ \hline
10	&60.45\\ \hline
\end{tabular}
\end{table} 

The relation between question meaningfulness assessments and correct answers is clearer when validation answers are taken into account. Figure \ref{fig:validation_bars} exhibits this relation for the different values of the evaluation (normalized to 0-1). As can be seen, when both real evaluations and validation answers are taken into account, F1-score is considerably higher. In addition, F1-score demonstrates a more consistent behaviour, increasing for smaller partitions of the test set. Around achieving 60\% of the dataset, F1-score oscilattes around 60, since all questions in the following partitions received the highest score.

\begin{figure*}[tp]
  \centering
  \includegraphics[width=0.65\textwidth]{images/validation_bars.png}
  \caption{Mean F1-score for different levels of question meaningfulness, based on true evaluations.}
  \label{fig:validation_bars}
\end{figure*}

\subsubsection{Regression filtering in Portuguese}
For the regression task in Portuguese, we translated the abstracts from English, to put the context in the same languages as the questions and answers.\footnote{Traditionally, it is thought that texts should be translated over queries, because their longer span provides more context and therefore better translations. This view had been put into question by \cite{saleh2020document}, who show that query translations may outperform document ones; even though the authors themselves admit the results cannot be easily generalized given its very specific domain. Anyway, given that query translation would mean, in our case, translating both a question and an answer, we opted for the approach in which only one piece of text would have to be translated by QA set (i.e., the abstract), even if it may not have the best performance individually.} Similarly to English, we considered two metrics for choosing a specific test: evaluation loss and R-squared training. In the case of Portuguese, there was a complete agreement between the two metrics. Evaluation loss ranged from 0.0696 to 0.1748, with an average value of 0.0958. R-squared validation went from -1.4590 to 0.0162, with an average value of -0.3493. Table \ref{tab:correlation_pt} brings the top results tests.

\begin{table}[h]
\caption{Top results of the regression tests in Portuguese}
\label{tab:correlation_pt}
\centering
\begin{tabular}{|l|c|c|c|}
\hline
\textbf{Ranking} & \textbf{Test number} & {\bf Validation loss}   & \textbf{R-squared} \\ \hline
1 & 423 & 0.0696 & 0.0162 \\ \hline
2 & 399 & 0.0700 & 0.0104 \\ \hline
3 & 327 & 0.0701 & 0.0103 \\ \hline
4 & 351 & 0.0709 & -0.0011 \\ \hline
5 & 403 & 0.0710 & -0.0020 \\ \hline
\end{tabular}
\end{table}

We chose test 423 [corpus = `un'; context = `abstract', data = `standard', balancing = `unbalanced'] as the input to the QA system, since it achieve the best results in both metrics. The fact that the best results was achieved using only the UN corpus, may be caused by the less technical aspect of these texts, something that may have facilitated the translation. Whereas in English, the best results was achieved when using only the question as input, in Portuguese this happened when just the abstract was used. In both cases, the combination question+abstract may have brought too much information, confusing the regressor.

As for the QA system itself, we used a Portuguese BERT base cased QA (Question Answering), finetuned on SQuAD
v1.1.\footnote{https://huggingface.co/pierreguillou/bert-base-cased-squad-v1.1-portuguese} The Portuguese version of SQuAD was made with the automatic translation of the original dataset performed with Google Cloud API.\footnote{https://github.com/nunorc/squad-v1.1-pt} No version of SQuAD 2.0 is available in Portuguese yet.

We compared the F1-score in three situations, similarly to what we did for English. First, we consider the quality of answers fine-tuned with the Portuguese version of SQuAD 1.1. Figure \ref{fig:prediction_pt} and Table \ref{tab:prediction_pt} show the results for this test. Compared to English, scores in Portuguese are much lower, something explainable by the contexts being translated with automatic tools. There is no clear trend in the graph either: F1-score diminishes until half of the dataset, then rises again, with a huge spike (probably due to randomness) in the last partition.

\begin{figure*}[tp]
  \centering
  \includegraphics[width=0.65\textwidth]{images/prediction_pt.png}
  \caption{F1-score for different partitions of test set for answers generated with SQuAD 1.1, based on predicted values.}
  \label{fig:prediction_pt}
\end{figure*}

\begin{table}[h]
\caption{F1-score for different partitions of test set for answers generated with SQuAD 1.1, based on predicted values}
\label{tab:prediction_pt}
\centering
\begin{tabular}{|l|c|}
\hline
{\bf Partition}   & \textbf{SQuAD 1.1}\\ \hline
100	&36.36\\ \hline
90	&35.53\\ \hline
80	&34.99\\ \hline
70	&34.40\\ \hline
60	&33.66\\ \hline
50	&34.23\\ \hline
40	&34.34\\ \hline
30	&35.29\\ \hline
20	&36.00\\ \hline
10	&48.42\\ \hline
\end{tabular}
\end{table}

Second, we consider the F1-score for different partitions of the dataset, based on true evaluations. Figure \ref{fig:real_label_pt} and Table \ref{tab:real_label_pt} show the results for this test. There is a much clearer trend here, with smaller partitions achieving higher F1-score values.

\begin{figure*}[tp]
  \centering
  \includegraphics[width=0.65\textwidth]{images/real_label_pt.png}
  \caption{F1-score for different partitions of test set for answers generated with SQuAD 1.1, based on true evaluations.}
  \label{fig:real_label_pt}
\end{figure*}

\begin{table}[h]
\caption{F1-score for different partitions of test set for answers generated with SQuAD 1.1, based on true evaluations.}
\label{tab:real_label_pt}
\centering
\begin{tabular}{|l|c|}
\hline
{\bf Partition}   & \textbf{SQuAD 1.1}\\ \hline
100	&36.36\\ \hline
90	&36.59\\ \hline
80	&37.93\\ \hline
70	&38.09\\ \hline
60	&37.60\\ \hline
50	&38.97\\ \hline
40	&39.20\\ \hline
30	&38.83\\ \hline
20	&40.57\\ \hline
10	&35.08\\ \hline
\end{tabular}
\end{table}


This fact offers evidence that the oscillating character or the F1-score for predicted values of question meaningfulness is largely due to the inability of our regressor to accurately measure that variable. This is confirmed by the correlation between the predicted values for question meaningfulness and the human evaluations. Table \ref{tab:correlation_pt} and Figure \ref{fig:correlation_pt}(a) present the mean value of the question evaluation for each value of the true label (normalized for the range 0-1). The Pearson correlation for this pair of variables gives a value of 0.0327, with a two-sided p-value of 0.6319. In other words, our regressor only slightly predicts the true meaningfulness of questions and even this without statistical significance. This weak correlation can be also seen in Figure \ref{fig:correlation_pt}(b).

\begin{figure*}[tp]
  \centering
  \includegraphics[width=0.9\textwidth]{images/correlation_pt.png}
  \caption{(a) Correlation between real labels and predictions (line plot); (b) Correlation between real labels and predictions (scatter plot)}
  \label{fig:correlation_pt}
\end{figure*}

\begin{table}[h]
\caption{Mean prediction for true question meaningfulness}
\label{tab:correlation_pt}
\centering
\begin{tabular}{|l|c|}
\hline
{\bf True label}   & \textbf{Mean prediction}\\ \hline
0	&83.60\\ \hline
0.25&	83.06\\ \hline
0.50&	83.03\\ \hline
0.75&	84.61\\ \hline
1	&83.82\\ \hline
\end{tabular}
\end{table}

As for English, the unbalancing among levels of question meaningfulness compromised the regressor's predictions in the test set (see Table \ref{tab:labels_size} and Figure \ref{fig:labels_size}). 

In the last test, we analyse the results of F1-score when partitions are based on the true assessment, and the validation answer is used as the comparison. Figure \ref{fig:real_label_pt} and Table \ref{tab:real_label_pt} show the results for this test. When validation answer were used together with true evaluations, F1-score achieved higher results. Figure \ref{fig:validation_answers_pt} and Table \ref{tab:validation_answers_pt} show the results for this last test. f1-score is higher for validation answers than for answers generated with SQuAD 1.1, which indicates points to shortcomings of this QA model, especially in Portuguese. Finally, there seems to be a negative correlation between a question's meaningfulness (as evaluated by a human) and the F1-score with the validation answer. 

\begin{figure*}[tp]
  \centering
  \includegraphics[width=0.65\textwidth]{images/validation_answers_pt.png}
  \caption{F1-score for different partitions of test set for validation answers, based on true evaluations.}
  \label{fig:validation_answers_pt}
\end{figure*}

\begin{table}[h]
\caption{F1-score for different partitions of test set for validation answers, based on true evaluations.}
\label{tab:validation_answers_pt}
\centering
\begin{tabular}{|l|c|}
\hline
{\bf Partition}   & \textbf{F1-score}\\ \hline
100	&51.70\\ \hline
90	&53.63\\ \hline
80	&55.23\\ \hline
70	&55.79\\ \hline
60	&56.40\\ \hline
50	&58.11\\ \hline
40	&59.57\\ \hline
30	&58.80\\ \hline
20	&56.19\\ \hline
10	&56.87\\ \hline
\end{tabular}
\end{table}

==> instrucoes.tex <==
\section{Tables}\label{sec5}

Tables can be inserted via the normal table and tabular environment. To put
footnotes inside tables you should use \verb+\footnotetext[]{...}+ tag.
The footnote appears just below the table itself (refer Tables~\ref{tab1} and \ref{tab2}). 
For the corresponding footnotemark use \verb+\footnotemark[...]+

\begin{table}[h]
\begin{center}
\begin{minipage}{174pt}
\caption{Caption text}\label{tab1}%
\begin{tabular}{@{}llll@{}}
\toprule
Column 1 & Column 2  & Column 3 & Column 4\\
\midrule
row 1    & data 1   & data 2  & data 3  \\
row 2    & data 4   & data 5\footnotemark[1]  & data 6  \\
row 3    & data 7   & data 8  & data 9\footnotemark[2]  \\
\botrule
\end{tabular}
\footnotetext{Source: This is an example of table footnote. This is an example of table footnote.}
\footnotetext[1]{Example for a first table footnote. This is an example of table footnote.}
\footnotetext[2]{Example for a second table footnote. This is an example of table footnote.}
\end{minipage}
\end{center}
\end{table}

\noindent
The input format for the above table is as follows:

%%=============================================%%
%% For presentation purpose, we have included  %%
%% \bigskip command. please ignore this.       %%
%%=============================================%%
\bigskip
\begin{verbatim}
\begin{table}[<placement-specifier>]
\begin{center}
\begin{minipage}{<preferred-table-width>}
\caption{<table-caption>}\label{<table-label>}%
\begin{tabular}{@{}llll@{}}
\toprule
Column 1 & Column 2 & Column 3 & Column 4\\
\midrule
row 1 & data 1 & data 2	 & data 3 \\
row 2 & data 4 & data 5\footnotemark[1] & data 6 \\
row 3 & data 7 & data 8	 & data 9\footnotemark[2]\\
\botrule
\end{tabular}
\footnotetext{Source: This is an example of table footnote. 
This is an example of table footnote.}
\footnotetext[1]{Example for a first table footnote.
This is an example of table footnote.}
\footnotetext[2]{Example for a second table footnote. 
This is an example of table footnote.}
\end{minipage}
\end{center}
\end{table}
\end{verbatim}
\bigskip
%%=============================================%%
%% For presentation purpose, we have included  %%
%% \bigskip command. please ignore this.       %%
%%=============================================%%

\begin{table}[h]
\begin{center}
\begin{minipage}{\textwidth}
\caption{Example of a lengthy table which is set to full textwidth}\label{tab2}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lcccccc@{\extracolsep{\fill}}}
\toprule%
& \multicolumn{3}{@{}c@{}}{Element 1\footnotemark[1]} & \multicolumn{3}{@{}c@{}}{Element 2\footnotemark[2]} \\\cmidrule{2-4}\cmidrule{5-7}%
Project & Energy & $\sigma_{calc}$ & $\sigma_{expt}$ & Energy & $\sigma_{calc}$ & $\sigma_{expt}$ \\
\midrule
Element 3  & 990 A & 1168 & $1547\pm12$ & 780 A & 1166 & $1239\pm100$\\
Element 4  & 500 A & 961  & $922\pm10$  & 900 A & 1268 & $1092\pm40$\\
\botrule
\end{tabular*}
\footnotetext{Note: This is an example of table footnote. This is an example of table footnote this is an example of table footnote this is an example of~table footnote this is an example of table footnote.}
\footnotetext[1]{Example for a first table footnote.}
\footnotetext[2]{Example for a second table footnote.}
\end{minipage}
\end{center}
\end{table}

In case of double column layout, tables which do not fit in single column width should be set to full text width. For this, you need to use \verb+\begin{table*}+ \verb+...+ \verb+\end{table*}+ instead of \verb+\begin{table}+ \verb+...+ \verb+\end{table}+ environment. Lengthy tables which do not fit in textwidth should be set as rotated table. For this, you need to use \verb+\begin{sidewaystable}+ \verb+...+ \verb+\end{sidewaystable}+ instead of \verb+\begin{table*}+ \verb+...+ \verb+\end{table*}+ environment. This environment puts tables rotated to single column width. For tables rotated to double column width, use \verb+\begin{sidewaystable*}+ \verb+...+ \verb+\end{sidewaystable*}+.

\begin{sidewaystable}
\sidewaystablefn%
\begin{center}
\begin{minipage}{\textheight}
\caption{Tables which are too long to fit, should be written using the ``sidewaystable'' environment as shown here}\label{tab3}
\begin{tabular*}{\textheight}{@{\extracolsep{\fill}}lcccccc@{\extracolsep{\fill}}}
\toprule%
& \multicolumn{3}{@{}c@{}}{Element 1\footnotemark[1]}& \multicolumn{3}{@{}c@{}}{Element\footnotemark[2]} \\\cmidrule{2-4}\cmidrule{5-7}%
Projectile & Energy	& $\sigma_{calc}$ & $\sigma_{expt}$ & Energy & $\sigma_{calc}$ & $\sigma_{expt}$ \\
\midrule
Element 3 & 990 A & 1168 & $1547\pm12$ & 780 A & 1166 & $1239\pm100$ \\
Element 4 & 500 A & 961  & $922\pm10$  & 900 A & 1268 & $1092\pm40$ \\
Element 5 & 990 A & 1168 & $1547\pm12$ & 780 A & 1166 & $1239\pm100$ \\
Element 6 & 500 A & 961  & $922\pm10$  & 900 A & 1268 & $1092\pm40$ \\
\botrule
\end{tabular*}
\footnotetext{Note: This is an example of table footnote this is an example of table footnote this is an example of table footnote this is an example of~table footnote this is an example of table footnote.}
\footnotetext[1]{This is an example of table footnote.}
\end{minipage}
\end{center}
\end{sidewaystable}

\section{Figures}\label{sec6}

As per the \LaTeX\ standards you need to use eps images for \LaTeX\ compilation and \verb+pdf/jpg/png+ images for \verb+PDFLaTeX+ compilation. This is one of the major difference between \LaTeX\ and \verb+PDFLaTeX+. Each image should be from a single input .eps/vector image file. Avoid using subfigures. The command for inserting images for \LaTeX\ and \verb+PDFLaTeX+ can be generalized. The package used to insert images in \verb+LaTeX/PDFLaTeX+ is the graphicx package. Figures can be inserted via the normal figure environment as shown in the below example:

%%=============================================%%
%% For presentation purpose, we have included  %%
%% \bigskip command. please ignore this.       %%
%%=============================================%%
\bigskip
\begin{verbatim}
\begin{figure}[<placement-specifier>]
\centering
\includegraphics{<eps-file>}
\caption{<figure-caption>}\label{<figure-label>}
\end{figure}
\end{verbatim}
\bigskip
%%=============================================%%
%% For presentation purpose, we have included  %%
%% \bigskip command. please ignore this.       %%
%%=============================================%%

\begin{figure}[h]%
\centering
\includegraphics[width=0.9\textwidth]{fig.eps}
\caption{This is a widefig. This is an example of long caption this is an example of long caption  this is an example of long caption this is an example of long caption}\label{fig1}
\end{figure}

In case of double column layout, the above format puts figure captions/images to single column width. To get spanned images, we need to provide \verb+\begin{figure*}+ \verb+...+ \verb+\end{figure*}+.


\backmatter

\bmhead{Supplementary information}

If your article has accompanying supplementary file/s please state so here. 

Authors reporting data from electrophoretic gels and blots should supply the full unprocessed scans for key as part of their Supplementary information. This may be requested by the editorial team/s if it is missing.

Please refer to Journal-level guidance for any specific requirements.

\bmhead{Acknowledgments}

Acknowledgments are not compulsory. Where included they should be brief. Grant or contribution numbers may be acknowledged.

Please refer to Journal-level guidance for any specific requirements.

\section*{Declarations}

Some journals require declarations to be submitted in a standardised format. Please check the Instructions for Authors of the journal to which you are submitting to see if you need to complete this section. If yes, your manuscript must contain the following sections under the heading `Declarations':

\begin{itemize}
\item Funding
\item Conflict of interest/Competing interests (check journal-specific guidelines for which heading to use)
\item Ethics approval 
\item Consent to participate
\item Consent for publication
\item Availability of data and materials
\item Code availability 
\item Authors' contributions
\end{itemize}

\noindent
If any of the sections are not relevant to your manuscript, please include the heading and write `Not applicable' for that section. 

%%===================================================%%
%% For presentation purpose, we have included        %%
%% \bigskip command. please ignore this.             %%
%%===================================================%%
\bigskip
\begin{flushleft}%
Editorial Policies for:

\bigskip\noindent
Springer journals and proceedings: \url{https://www.springer.com/gp/editorial-policies}

\bigskip\noindent
Nature Portfolio journals: \url{https://www.nature.com/nature-research/editorial-policies}

\bigskip\noindent
\textit{Scientific Reports}: \url{https://www.nature.com/srep/journal-policies/editorial-policies}

\bigskip\noindent
BMC journals: \url{https://www.biomedcentral.com/getpublished/editorial-policies}
\end{flushleft}
For sample purpose, we have included the width of images in the optional argument of \verb+\includegraphics+ tag. Please ignore this. 

==> sections/future_work.tex <==
1. Treinar o UnifiedQA para todas as tarefas

2. Conduzir avaliações humanas na tarefa de MCQA

3. Fazer a seção de MCQA em português
